A novel search strategy for right-handed charged gauge bosons at the Large Hadron Collider

We explore the potential of the Large Hadron Collider (LHC) in detecting a signal originating from the production of a heavy $SU(2)_R$ charged gauge boson that then decays into a top-bottom quark pair via the mediation of a right-handed neutrino, $p p \to W_R \to N_R \ell \to (\ell' t b)\ell$. Such a channel, that we study in the context of the minimal Left-Right Symmetric Model, contrasts with conventional smoking-gun signatures targeted experimentally and phenomenologically in which only light quarks are involved. We propose a selection strategy aimed at extracting such a top-bottom signal and we estimate the resulting sensitivity of the LHC to the model. Our results demonstrate the potential impact of such a search and we therefore urge the experimental collaborations to carry out a similar analysis in the light of present and future data.

==> Sections/cms_exo_17_011.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The CMS-EXO-17-011 search for $W_R$ in the $\ell\ell jj$ channel}
\label{sec:CMS-EXO-17-011}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Event selection}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Events are selected if they contain at least two high-$p_T$ leptons and two jets. The leptons and the jets with the largest $p_T$ are selected to reconstruct the $W_R$ candidates. The leading (subleading) leptons are required to have $p_T > 60$~($53$) GeV and to be within the detector acceptance ($|\eta| < 2.4$). On the other hand, electrons are rejected if they lie in the range ($1.444 < |\eta| < 1.566$), which correspond to the transition  region between the barrel and endcap section s of the Electromagnetic Calorimeter (ECAL).  Muons for which the sum of the $p_T$ of additional tracks that originate from the primary vertex  inside a cone of $R < 0.3$ around the muon is more than $10\%$ are removed. This selection is important to suppress the contribution of muons that are originated from hadron decays or pion punch-thorugh in jets. On the other hand, electrons are required to be isolated. We require that the sum of the $p_T$ of all tracks inside a cone of $R < 0.3$ centered around the electron axis, to be below than $5$ GeV. The two jet candidates must each have $p_T > 40$ GeV and be within $|\eta| < 2.4$. To avoid having reconstructed leptons overlap jets, we impose a $\Delta R > $ 0.4 requirement between all jets and leptons. We focus our search on a region of phase-space where the signal is expected to appear. This signal region applies to events with two leptons with the same flavor and two jets. The invariant mass of the dilepton system must be above $200$ GeV, to avoid contamination from resonant Z boson production. The $m_{\ell \ell jj}$ must be greater than $600$ GeV to ensure that all the kinematic requirements on the candidates are fully efficient. The definition of all the cuts is shown in table \ref{tab:cuts:definition}. 

\begin{table}[t!]
\setlength\tabcolsep{2pt}
  \begin{center}
    \begin{tabular}{ll}
      \toprule
      Cut & Definition \\
      \midrule
      Initial & Number of initial events normalised to the total luminosity
      ($35.9~{\rm fb}^{-1}$). \\
      \midrule 
      $N_{\rm jets} \geq 2$ & At least two jets with $p_T > 25~{\rm GeV}$ and $|\eta| < 2.4$ \\ 
      \midrule
      $N_{\ell} \geq 2$ & At least two isolated charged leptons \\
      \midrule 
      $p_T({\rm jets}) > 40$ GeV & The $p_T$ of the leading and subleading jets should be larger than $40$ GeV \\ 
      \midrule 
      $p_T^{\ell_1} > 60~{\rm GeV}$ & the $p_T$ of the leading~(subleading) lepton should be larger than $60$~($53$) GeV \\
      $p_T^{\ell_2} > 53~{\rm GeV}$ & \\
      \midrule 
      $\Delta R_{\ell j} > 0.4$ & Lepton and Jets should be separated by at least $\Delta R > 0.4$.  \\ 
      \midrule 
      $m_{\ell \ell} > 200~{\rm GeV}$ & The invariant mass of the dilepton system should be larger than 200 GeV. \\
      \midrule 
      $m_{\ell \ell jj} > 600~{\rm GeV}$ & The invariant mass of the $W_R$ candidate should be larger than $600$ GeV. \\ 
 \bottomrule
    \end{tabular}
  \end{center}
  \caption{Definitions of the different cuts used in this analysis}
  \label{tab:cuts:definition}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Momentum smearing and particle reconstruction efficiencies}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The modeling of the particle smearing and reconstruction efficiencies in \textsc{MadAnalysis}~5 is based on the SFS module \cite{Araz:2020lnp} where the default parametrisations are used (the detector card is shipped with the newest version of \textsc{MadAnalysis}~5). For convenience, I show the momentum smearing and particle reconstruction efficiencies used in this analysis.  
We start with the electron reconstruction efficiency. In the default options, it used to be equal to $0$ for $p_T^e < 10~{\rm GeV}$ and $0.95$ otherwise. 
\paragraph{{\bf Electron Momentum Smearing}}
\begin{eqnarray}
\mathcal{S}_e = \begin{cases}
		\sqrt{0.03^2 + (1.3~p_{T,e})^2 / 10^{6}} & \mathrm{if}\ |\eta| \leq 0.5 ~{\rm and}~p_{T,e} > 0.1~{\rm GeV}, \\
		\sqrt{0.05^2 + (1.7~p_{T,e})^2 / 10^{6}} & \mathrm{if}\,  0.5 < |\eta| \leq 1.5 ~{\rm and}~p_{T,e} > 0.1~{\rm GeV}, \\ 
		\sqrt{0.15^2 + (3.1~p_{T,e})^2 / 10^{6}} & \mathrm{if}\,  1.5 < |\eta| \leq 2.5 ~{\rm and}~p_{T,e} > 0.1~{\rm GeV}, 
		\end{cases}
\end{eqnarray}

\paragraph{{\bf Muon Momentum Smearing}}
\begin{eqnarray}
\mathcal{S}_\mu = \begin{cases}
		\sqrt{0.01^2 + (p_{T,\mu})^2 / 10^{8}} & \mathrm{if}\ |\eta| \leq 0.5 ~{\rm and}~p_{T,\mu} > 0.1~{\rm GeV}, \\
		\sqrt{0.015^2 + (1.5~p_{T,\mu})^2 / 10^{8}} & \mathrm{if}\,  0.5 < |\eta| \leq 1.5 ~{\rm and}~p_{T,\mu} > 0.1~{\rm GeV}, \\ 
		\sqrt{0.025^2 + (3.5~p_{T,\mu})^2 / 10^{8}} & \mathrm{if}\,  1.5 < |\eta| \leq 2.5 ~{\rm and}~p_{T,\mu} > 0.1~{\rm GeV}, 
		\end{cases}
\end{eqnarray}

\paragraph{{\bf Muon Reconstruction Efficiency}}
\begin{eqnarray}
\mathcal{E}_\mu = \begin{cases}
        0 & {\rm if}\ p_T < 10~{\rm GeV~and}~ |\eta| > 2.4, \\
        0.891 & {\rm if}\ 10~{\rm GeV} < p_T \leq 1000~{\rm GeV~and}~ |\eta| \leq 2.4, \\
        0.891~\exp(0.5 - 5 \times 10^{-4} p_T) & {\rm if}\ 10~{\rm GeV} < p_T \leq 1000~{\rm GeV~and}~|\eta| \leq 1.5, \\
        0.882 & {\rm if}\ 10~{\rm GeV} < p_T \leq 1000~{\rm GeV~and}~1.5 < |\eta| \leq 2.4, \\
        0.882~\exp(0.5 - 5 \times 10^{-4} p_T) & {\rm if}\ p_T > 1000~{\rm GeV~and}~ |\eta| \leq 2.4, \\
	\end{cases}
\end{eqnarray}

\paragraph{{\bf Jet reconstruction efficiency}}
\begin{eqnarray}
\mathcal{E}_j = \begin{cases}
	 0.925 & \mathrm{if}\ |\eta| \leq 1.5, \\
	 0.875 & \mathrm{if}\,  1.5 < |\eta| \leq 2.5, \\ 
	 0.80  & \mathrm{if}\,  2.5 < |\eta|, \\ 
	\end{cases}
\end{eqnarray}

\paragraph{{\bf Jet Momentum Smearing}}
\begin{eqnarray}
\mathcal{S}_j = \begin{cases}
	 \sqrt{0.06^2 + (1.3 \times p_T / 10^3)^2} & \mathrm{if}\ |\eta| \leq 0.5, \\
	 \sqrt{0.10^2 + (1.7 \times p_T / 10^3)^2} & \mathrm{if}\ 0.5 < |\eta| \leq 1.5, \\ 
	 \sqrt{0.25^2 + (3.1 \times p_T / 10^3)^2} & \mathrm{if}\ 1.5 < |\eta| \leq 2.5, \\
	\end{cases}
\end{eqnarray}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{The invariant mass of the $\ell\ell jj$ system}

 In figure \ref{fig:mlljj:SR}, we display the invariant mass of the $W_R$ candidate in the SR that satisfy all the cuts defined in table \ref{tab:cuts:definition} for $M_{W_R} = 4000$ GeV and $M_{N_R} = 2000$ GeV. The CMS simulation is shown in black and the result of \textsc{MadAnalysis}~5 is shown in red for the electron channel (left) and the muon channel (right).  
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.49\linewidth]{Figures/mlljj_ee_MWR_4000.pdf}
    \hfill 
    \includegraphics[width=0.49\linewidth]{Figures/mlljj_mm_MWR_4000.pdf}
    \caption{The $m_{\ell \ell jj}$ distribution in the signal region for the electron (left) and muon (right) channel. The black dots show the results of the CMS simulations \cite{CMS:2018agk} while the red line corresponds to the \textsc{MadAnalysis} result.}
    \label{fig:mlljj:SR}
\end{figure}

\subsubsection{Cutflow tables}
The cutflow tables for the analysis are shown in tables \ref{tab:cutflow:electrons} (electron channel) and \ref{tab:cutflow:muons} (muon channel) for three $W_R$ masses: $2200$, $2800$ and $3600$ GeV. The $N_R$ is assumed to have a mass of $M_{W_R} / 2$ for each mass scenario. For each case, we show the number of events normalised to the luminosity of $35.9$ fb$^{-1}$ and the corresponding cross section computed at LO and the acceptance times the efficiency defined as 
\begin{eqnarray}
\epsilon = N_{i} / N_{i-1},
\end{eqnarray}
where $N_k$ corresponds to the number of events surviving the cut $k$. 

\begin{table}[!t]
  \begin{center}
    \renewcommand{\arraystretch}{1.}
    \begin{tabular}{l||cc|cc|cc}
      & \multicolumn{2}{c|}{$M_{W_R}=2200$} & \multicolumn{2}{c|}{$M_{W_R}=2800$} & \multicolumn{2}{c}{$M_{W_R}=3600$}  \\ \hline \hline
      & Events & $\varepsilon$ & Events & $\varepsilon$ & Events & $\varepsilon$  \\ \hline
      Initial                                 & 951.0 & -  & 215.5 & - & 53.8 & -  \\
      $N_{\rm jets} \geq 2$                   & 946.3 $ \pm $ 0.7 & 0.995 & 214.7 $ \pm $ 0.1 & 0.996 & 53.6 $ \pm $ 0.0 & 0.996  \\
      $N_{\ell} \geq 2$                       & 418.8 $ \pm $ 3.1 & 0.443 & 93.0 $ \pm $ 0.7 & 0.433 & 23.1 $ \pm $ 0.2 & 0.430 \\
      $p_{T}({\rm jets}) > 40~{\rm GeV}$      & 418.4 $ \pm $ 3.1 & 0.999 & 92.8 $ \pm $ 0.7 & 0.998 & 23.1 $ \pm $ 0.2 & 1.000  \\
      $p_{T}^{\ell_1} > 60~{\rm GeV}, p_{T}^{\ell_2} > 53~{\rm GeV}$& 411.4 $ \pm $ 3.1 & 0.983 & 91.7 $ \pm $ 0.7 & 0.987 & 22.9 $ \pm $ 0.2 & 0.994 \\
      $\Delta R_{\ell j} > 0.4$               & 411.4 $ \pm $ 3.1 & 1.000 & 91.7 $ \pm $ 0.7 & 1.000 & 22.9 $ \pm $ 0.2 & 1.000 \\
      $m_{\ell \ell} > 200~{\rm GeV}$         & 403.2 $ \pm $ 3.1 & 0.980 & 90.9 $ \pm $ 0.7 & 0.991 & 22.8 $ \pm $ 0.2 & 0.994  \\
      $m_{\ell \ell j j} > 600~{\rm GeV}$     & 402.8 $ \pm $ 3.1 & 0.999 & 90.8 $ \pm $ 0.7 & 1.000 & 22.8 $ \pm $ 0.2 & 1.000 \\
      $m_{\ell \ell jj} \in [1960, 2810]~{\rm GeV}$& 254.3 $ \pm $ 2.2 & 0.631 & 25.6 $ \pm $ 0.2 & 0.282 & 1.9 $ \pm $ 0.0 & 0.083 \\
      $m_{\ell \ell jj} \in [2530, 3840]~{\rm GeV}$& 153.3 $ \pm $ 1.4 & 0.381 & 64.9 $ \pm $ 0.5 & 0.714 & 9.6 $ \pm $ 0.1 & 0.420 \\
      $m_{\ell \ell jj} \in [3250, 5170]~{\rm GeV}$& 24.8 $ \pm $ 0.2 & 0.062 & 32.7 $ \pm $ 0.3 & 0.360 & 16.6 $ \pm $ 0.1 & 0.728  
    \end{tabular}
    \caption{Cut flow table for the $ee$ channel. Here we show three cases: $M_{W_R} = 2200, 2800, 3600$ GeV while $M_{N_R} = M_{W_R} / 2$. More details can be found in the text.}
    \label{tab:cutflow:electrons}
  \end{center}
\end{table}


%% mm_mlljj_1860_2800

\begin{table}[!h]
  \begin{center}
    \renewcommand{\arraystretch}{1.}
    \begin{tabular}{l||cc|cc|cc}
      & \multicolumn{2}{c|}{$M_{W_R}=2200$} & \multicolumn{2}{c|}{$M_{W_R}=2800$} & \multicolumn{2}{c}{$M_{W_R}=3600$} \\ \hline\hline
      & Events & $\varepsilon$ & Events & $\varepsilon$ & Events & $\varepsilon$ \\ \hline
      Initial                                 & 884.9 & -  & 215.5 & -  & 53.8 & - \\
      $N_{\rm jets} \geq 2$                   & 806.9 $ \pm $ 2.4 & 0.912 & 200.3 $ \pm $ 0.5 & 0.929 & 50.5 $ \pm $ 0.1 & 0.937  \\
      $N_{\ell} \geq 2$                       & 570.1 $ \pm $ 3.4 & 0.707 & 140.9 $ \pm $ 0.8 & 0.703 & 33.6 $ \pm $ 0.2 & 0.665  \\
      $p_{T}({\rm jets}) > 40~{\rm GeV}$      & 530.9 $ \pm $ 3.4 & 0.931 & 132.9 $ \pm $ 0.8 & 0.943 & 32.0 $ \pm $ 0.2 & 0.952 \\
      $p_{T}^{\ell_1} > 60~{\rm GeV}, p_{T}^{\ell_2} > 53~{\rm GeV}$& 520.1 $ \pm $ 3.3 & 0.980 & 131.5 $ \pm $ 0.8 & 0.989 & 31.7 $ \pm $ 0.2 & 0.992  \\
      $\Delta R_{\ell j} > 0.4$               & 520.1 $ \pm $ 3.3 & 1.000 & 131.5 $ \pm $ 0.8 & 1.000 & 31.7 $ \pm $ 0.2 & 1.000 \\
      $m_{\ell \ell} > 200~{\rm GeV}$         & 511.1 $ \pm $ 3.3 & 0.983 & 130.0 $ \pm $ 0.8 & 0.989 & 31.5 $ \pm $ 0.2 & 0.994 \\
      $m_{\ell \ell j j} > 600~{\rm GeV}$     & 510.9 $ \pm $ 3.3 & 1.000 & 130.0 $ \pm $ 0.8 & 1.000 & 31.5 $ \pm $ 0.2 & 1.000 \\
      $m_{\ell \ell jj} \in [1860, 2800]~{\rm GeV}$& 382.5 $ \pm $ 2.9 & 0.749 & 104.7 $ \pm $ 0.8 & 0.805  & 4.6 $ \pm $ 0.0 & 0.144 \\
      $m_{\ell \ell jj} \in [2430, 3930]~{\rm GeV}$& 25.1 $ \pm $ 0.2 & 0.049 & 89.3 $ \pm $ 0.7 & 0.687 & 28.5 $ \pm $ 0.2 & 0.904 \\
      $m_{\ell \ell jj} \in [3190, 5500]~{\rm GeV}$& 2.4 $ \pm $ 0.0 & 0.005 & 2.9 $ \pm $ 0.0 & 0.022 & 19.5 $ \pm $ 0.2 & 0.618 \\
    \end{tabular}
    \caption{Cut flow table for the $\mu\mu$ channel. Here we show three cases: $M_{W_R} = 2200, 2800, 3600$ GeV while $M_{N_R} = M_{W_R} / 2$. More details can be found in the text.}
    \label{tab:cutflow:muons}
  \end{center}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Event yields in the SRs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In table \ref{tab:SR:ee:mm}, we show the comparison between the results of \textsc{MadAnalysis}~5 and CMS for different $W_R$ masses and different mass windows. To better quantify the discrepancies we compute the quantity $\delta$ defined by

\begin{eqnarray}
\delta = 100 \times \bigg|1 - \frac{n_{\rm MA5}}{n_{\rm CMS}}\bigg|,
\end{eqnarray}
where $n_{\rm MA5}$~($n_{\rm CMS}$) refers to the number of events obtained ~(reported on) by \textsc{MadAnalysis}~5~(CMS) in the mass window $[m_{\ell \ell jj}^{\rm min}, m_{\ell \ell jj}^{\rm max}]$ for a $W_R$ boson with mass $M_{W_R}$. 

\begin{table}[t!]
\setlength\tabcolsep{8pt}
  \begin{center}
    \begin{tabular}{llll}
      \toprule
      $M_{W_R}$~($[m_{\ell \ell jj}^{\rm min}, m_{\ell \ell jj}^{\rm max}]$) & \textsc{MadAnalysis}~5 & CMS & $\delta~[\%]$ \\
      \midrule
      \multicolumn{4}{c}{Electron Channel} \\
      \midrule
      $2200$~([$1950, 2810$]) & $325.3 \pm 2.7$ & $474.0 \pm 3.7 \pm 44.7$ & $31.38$ \\
      $2800$~([$2530, 3840$]) & $79.1 \pm 0.6$ & $114.1 \pm 0.9 \pm 10.6$ & $30.67$ \\
      $3600$~([$3250, 5170$]) & $12.9 \pm 0.1$ & $19.2 \pm 0.2 \pm 1.8$ & $32.96$ \\
      \midrule 
      \multicolumn{4}{c}{Muon Channel} \\
      \midrule 
      $2200$~([$1860, 2800$]) & $628.1 \pm 4.0$ & $744.0 \pm 4.7 \pm 47.5$ & $15.57$ \\ 
      $2800$~([$2430, 3930$]) & $144.0 \pm 0.9$ & $177.0 \pm 1.1 \pm 13.1$ & $18.6$ \\
      $3600$~([$3190, 5500$]) & $22.3 \pm 0.1$ & $29.2 \pm 0.2 \pm 2.6$ & $23.56$ \\ 
      \bottomrule
    \end{tabular}
  \end{center}
  \caption{Comparison between the CMS results (table 4 of \cite{CMS:2018agk}) for different $W_R$ masses and different signal regions.}
  \label{tab:SR:ee:mm}
\end{table}


==> Sections/cms_exo_20_002.tex <==
\section{CMS-EXO-20-002}

\begin{table}[h]
  \begin{center}
    \renewcommand{\arraystretch}{1.}
    \begin{tabular}{l||cc|ccc}
      & \multicolumn{2}{c|}{CMS} & \multicolumn{3}{c}{MadAnalysis5} \\ \hline\hline
      & Events & $\varepsilon$ & Events & $\varepsilon$ & $\delta$ [\%]\\ \hline
      Initial                                 & 586.6 & -  & 587.2 & - & - \\
      $N_{\ell} \geq 2~{\rm with}~p_{T}^{\ell} > 60~(53)~{\rm GeV}$& 494.5 $ \pm $ 0.0 & 0.843 & 498.6 $ \pm $ 1.9 & 0.849 & 0.7 \\
      $\geq 2~{\rm AK4~jets~with}~p_T > 40~{\rm GeV}$& 473.2 $ \pm $ 0.0 & 0.957 & 450.6 $ \pm $ 2.2 & 0.904 & 5.6 \\
      $\Delta R > 0.4~{\rm between~all~pairs~of~objects}$& 443.1 $ \pm $ 0.0 & 0.936 & 450.6 $ \pm $ 2.2 & 1.000 & 6.8 \\
      $m_{\ell\ell} > 200~{\rm GeV}$          & 420.8 $ \pm $ 0.0 & 0.950 & 447.3 $ \pm $ 2.2 & 0.993 & 4.5 \\
      $m_{\ell\ell jj} > 800~{\rm GeV}$       & 420.7 $ \pm $ 0.0 & 1.000 & 447.2 $ \pm $ 2.2 & 1.000 & 0.0 \\
      $m_{\ell\ell} > 400~{\rm GeV}~(\mu\mu)$ & 407.3 $ \pm $ 0.0 & 0.968 & 431.6 $ \pm $ 2.2 & 0.965 & 0.3 \\
    \end{tabular}
    \caption{Cut flow for the $\mu\mu$ + jets for $(M_{W_R}, M_{N_R}) = (3000, 1400)$ GeV.}
  \end{center}
\end{table}

\begin{table}[h]
  \begin{center}
    \renewcommand{\arraystretch}{1.}
    \begin{tabular}{l||cc|ccc}
      & \multicolumn{2}{c|}{CMS} & \multicolumn{3}{c}{MadAnalysis5} \\ \hline\hline
      & Events & $\varepsilon$ & Events & $\varepsilon$ & $\delta$ [\%]\\ \hline
      Initial                                 & 57.6 & -  & 57.6 & - & - \\
      $N_{\ell} \geq 2~{\rm with}~p_{T}^{\ell} > 60~(53)~{\rm GeV}$& 49.8 $ \pm $ 0.0 & 0.864 & 45.2 $ \pm $ 0.2 & 0.786 & 9.1 \\
      $\geq 2~{\rm AK4~jets~with}~p_T > 40~{\rm GeV}$& 48.4 $ \pm $ 0.0 & 0.971 & 41.8 $ \pm $ 0.2 & 0.925 & 4.8 \\
      $\Delta R > 0.4~{\rm between~all~pairs~of~objects}$& 45.4 $ \pm $ 0.0 & 0.940 & 41.8 $ \pm $ 0.2 & 1.000 & 6.4 \\
      $m_{\ell\ell} > 200~{\rm GeV}$          & 43.5 $ \pm $ 0.0 & 0.957 & 41.7 $ \pm $ 0.2 & 0.997 & 4.2 \\
      $m_{\ell\ell jj} > 800~{\rm GeV}$       & 43.5 $ \pm $ 0.0 & 1.000 & 41.7 $ \pm $ 0.2 & 1.000 & 0.0 \\
      $m_{\ell\ell} > 400~{\rm GeV}~(\mu\mu)$ & 42.8 $ \pm $ 0.0 & 0.985 & 40.7 $ \pm $ 0.2 & 0.977 & 0.8 \\
    \end{tabular}
    \caption{Cut flow for the $\mu\mu$ + jets for $(M_{W_R}, M_{N_R}) = (4000, 2000)$ GeV.}
  \end{center}
\end{table}

\begin{table}[h]
  \begin{center}
    \renewcommand{\arraystretch}{1.}
    \begin{tabular}{l||cc|ccc}
      & \multicolumn{2}{c|}{CMS} & \multicolumn{3}{c}{MadAnalysis5} \\ \hline\hline
      & Events & $\varepsilon$ & Events & $\varepsilon$ & $\delta$ [\%]\\ \hline
      Initial                                 & 5.9 & -  & 5.9 & - & - \\
      $N_{\ell} \geq 2~{\rm with}~p_{T}^{\ell} > 60~(53)~{\rm GeV}$& 5.1 $ \pm $ 0.0 & 0.858 & 4.4 $ \pm $ 0.0 & 0.749 & 12.7 \\
      $\geq 2~{\rm AK4~jets~with}~p_T > 40~{\rm GeV}$& 5.0 $ \pm $ 0.0 & 0.984 & 4.1 $ \pm $ 0.0 & 0.923 & 6.2 \\
      $\Delta R > 0.4~{\rm between~all~pairs~of~objects}$& 4.7 $ \pm $ 0.0 & 0.940 & 4.1 $ \pm $ 0.0 & 1.000 & 6.4 \\
      $m_{\ell\ell} > 200~{\rm GeV}$          & 4.5 $ \pm $ 0.0 & 0.960 & 4.1 $ \pm $ 0.0 & 0.997 & 3.9 \\
      $m_{\ell\ell jj} > 800~{\rm GeV}$       & 4.5 $ \pm $ 0.0 & 1.000 & 4.1 $ \pm $ 0.0 & 1.000 & 0.0 \\
      $m_{\ell\ell} > 400~{\rm GeV}~({\rm \mu\mu})$& 4.5 $ \pm $ 0.0 & 0.991 & 4.0 $ \pm $ 0.0 & 0.982 & 0.9 \\
    \end{tabular}
    \caption{Cut flow for the $\mu\mu$ + jets for $(M_{W_R}, M_{N_R}) = (5000, 3000)$ GeV.}
  \end{center}
\end{table}

\begin{table}[h]
  \begin{center}
    \renewcommand{\arraystretch}{1.}
    \begin{tabular}{l||cc|ccc}
      & \multicolumn{2}{c|}{CMS} & \multicolumn{3}{c}{MadAnalysis5} \\ \hline\hline
      & Events & $\varepsilon$ & Events & $\varepsilon$ & $\delta$ [\%]\\ \hline
      Initial                                 & 1175.4 & -  & 1174.4 & - & - \\
      $N_{\ell} \geq 2~{\rm with}~p_{T}^{\ell} > 60~(53)~{\rm GeV}$& 379.5 $ \pm $ 0.0 & 0.323 & 363.5 $ \pm $ 3.0 & 0.309 & 4.1 \\
      $\geq 2~{\rm AK4~jets~with}~p_T > 40~{\rm GeV}$& 363.1 $ \pm $ 0.0 & 0.957 & 363.0 $ \pm $ 3.0 & 0.999 & 4.4 \\
      $\Delta R > 0.4~{\rm between~all~pairs~of~objects}$& 355.4 $ \pm $ 0.0 & 0.979 & 363.0 $ \pm $ 3.0 & 1.000 & 2.2 \\
      $m_{\ell\ell} > 200~{\rm GeV}$          & 335.6 $ \pm $ 0.0 & 0.944 & 358.3 $ \pm $ 3.0 & 0.987 & 4.5 \\
      $m_{\ell\ell jj} > 800~{\rm GeV}$       & 335.6 $ \pm $ 0.0 & 1.000 & 357.1 $ \pm $ 3.0 & 0.997 & 0.3 \\
      $m_{\ell\ell} > 400~{\rm GeV}~({\rm ee})$& 324.1 $ \pm $ 0.0 & 0.966 & 339.5 $ \pm $ 2.9 & 0.951 & 1.6 \\
    \end{tabular}
    \caption{mll e channel 400 infinity Some notes here for the caption }
  \end{center}
\end{table}


\begin{table}[h]
  \begin{center}
    \renewcommand{\arraystretch}{1.}
    \begin{tabular}{l||cc|ccc}
      & \multicolumn{2}{c|}{CMS} & \multicolumn{3}{c}{MadAnalysis5} \\ \hline\hline
      & Events & $\varepsilon$ & Events & $\varepsilon$ & $\delta$ [\%]\\ \hline
      Initial                                 & 115.2 & -  & 115.2 & - & - \\
      $N_{\ell} \geq 2~{\rm with}~p_{T}^{\ell} > 60~(53)~{\rm GeV}$& 37.2 $ \pm $ 0.0 & 0.322 & 32.9 $ \pm $ 0.3 & 0.285 & 11.5 \\
      $\geq 2~{\rm AK4~jets~with}~p_T > 40~{\rm GeV}$& 36.0 $ \pm $ 0.0 & 0.969 & 32.7 $ \pm $ 0.3 & 0.996 & 2.8 \\
      $\Delta R > 0.4~{\rm between~all~pairs~of~objects}$& 35.1 $ \pm $ 0.0 & 0.974 & 32.7 $ \pm $ 0.3 & 1.000 & 2.6 \\
      $m_{\ell\ell} > 200~{\rm GeV}$          & 33.2 $ \pm $ 0.0 & 0.947 & 32.5 $ \pm $ 0.3 & 0.993 & 4.8 \\
      $m_{\ell\ell jj} > 800~{\rm GeV}$       & 33.2 $ \pm $ 0.0 & 1.000 & 32.5 $ \pm $ 0.3 & 0.999 & 0.1 \\
      $m_{\ell\ell} > 400~{\rm GeV}~({\rm ee})$& 32.5 $ \pm $ 0.0 & 0.979 & 31.4 $ \pm $ 0.3 & 0.966 & 1.3 \\
    \end{tabular}
    \caption{mll e channel 400 infinity Some notes here for the caption }
  \end{center}
\end{table}

\begin{table}[h]
  \begin{center}
    \renewcommand{\arraystretch}{1.}
    \begin{tabular}{l||cc|ccc}
      & \multicolumn{2}{c|}{CMS} & \multicolumn{3}{c}{MadAnalysis5} \\ \hline\hline
      & Events & $\varepsilon$ & Events & $\varepsilon$ & $\delta$ [\%]\\ \hline
      Initial                                 & 11.8 & -  & 11.8 & - & - \\
      $N_{\ell} \geq 2~{\rm with}~p_{T}^{\ell} > 60~(53)~{\rm GeV}$& 3.8 $ \pm $ 0.0 & 0.317 & 3.1 $ \pm $ 0.0 & 0.264 & 16.9 \\
      $\geq 2~{\rm AK4~jets~with}~p_T > 40~{\rm GeV}$& 3.7 $ \pm $ 0.0 & 0.987 & 3.1 $ \pm $ 0.0 & 0.999 & 1.3 \\
      $\Delta R > 0.4~{\rm between~all~pairs~of~objects}$& 3.6 $ \pm $ 0.0 & 0.968 & 3.1 $ \pm $ 0.0 & 1.000 & 3.4 \\
      $m_{\ell\ell} > 200~{\rm GeV}$          & 3.4 $ \pm $ 0.0 & 0.947 & 3.1 $ \pm $ 0.0 & 0.997 & 5.3 \\
      $m_{\ell\ell jj} > 800~{\rm GeV}$       & 3.4 $ \pm $ 0.0 & 1.000 & 3.1 $ \pm $ 0.0 & 1.000 & 0.0 \\
      $m_{\ell\ell} > 400~{\rm GeV}~({\rm ee})$& 3.4 $ \pm $ 0.0 & 0.988 & 3.0 $ \pm $ 0.0 & 0.974 & 1.4 \\
    \end{tabular}
    \caption{mll e channel 400 infinity Some notes here for the caption }
  \end{center}
\end{table}
